Improving Image Captioning by Mimicking Human Reformulation Feedback at Inference-time

Incorporating automatically predicted human feedback into the process of training generative models has attracted substantial recent interest, while feedback at inference time has received less attention. The typical feedback at training time, i.e., preferences of choice given two samples, does not naturally transfer to the inference phase. We introduce a novel type of feedback -- caption reformulations -- and train models to mimic reformulation feedback based on human annotations. Our method does not require training the image captioning model itself, thereby demanding substantially less computational effort. We experiment with two types of reformulation feedback: first, we collect a dataset of human reformulations that correct errors in the generated captions. We find that incorporating reformulation models trained on this data into the inference phase of existing image captioning models results in improved captions, especially when the original captions are of low quality. We apply our method to non-English image captioning, a domain where robust models are less prevalent, and gain substantial improvement. Second, we apply reformulations to style transfer. Quantitative evaluations reveal state-of-the-art performance on German image captioning and English style transfer, while human validation with a detailed comparative framework exposes the specific axes of improvement.

==> literature_review.tex <==
\citet{Shen_2019_ICCV} propose a captioning model that learns improved captions by asking questions. The model consists of three modules: a captioner, a decision maker that decides when and about what to ask questions, and a question generator. During training, the captioner generates a caption given an image, and the decision maker decides which word to ask a question about (or none of the words). The question generator then generates a corresponding question that is answered by a human. The answer should be one word, and the model replaces the corresponding word in the caption. For example:
\\\\
\textbf{Caption:} \emph{A dog is sitting on a bench}.
\\
\textbf{Decision maker decides to ask about} \emph{bench}.
\\
\textbf{Question:} \emph{What is the dog sitting on?}
\\
\textbf{The human answers:} \emph{car}.
\\
\textbf{Final caption:} \emph{A dog sitting on a car}.
\\

The human then evaluates both the original and the new caption. No questions are asked during test.

\citet{jia2020icap} introduce a captioning framework where a human start generating the caption and the model completes it, or the human generates a caption and the model reformulates it, until the human approves the generated caption.

\citet{hartmann_2022} propose to use reformulations in addition to annotations of the location of the error in the image, but only after the model is trained, as additional training. Their publication seems like a research plan rather than a paper, with no results published, but still \citet{goyal2022performance} cite them as if they published results.

Most similar to our work is that of \citet{ling2017teaching}. They trained a captioning model using static ground-truth captions and then used a snapshot of the model to generate captions for new images. Their model is unique in that it not only outputs words, but also splits the generated sentence into phrases. After training, they collected human feedback on the captions, instructing the annotators to highlight the word/phrase containing the error, write feedback in natural language, and correct the selected word/phrase. First, they trained a model that, given a model-generated caption, feedback, and a corrected caption, predicts whether the new caption is correct conditioned on the feedback. Next, they compared models trained with ground-truth captions only, models trained with GT captions in addition to corrected captions, and models trained with GT and corrected captions in addition to model-generated captions labeled correct, and showed that each addition improved standard metrics (BLEU and ROUGE -L). Their work differs from ours in several respects: First, they began providing human feedback late in the training process, after the model had been trained on many instances. Second, the annotators were asked to identify only a single error in a specific word or phrase (local errors): this is only possible because the quality of the captions is already good, due to the first difference. This makes the annotation process more difficult and limits the feedback to local errors. Third, this is a 2017 study based on RNNs and not Transformers; the results obtained could differ for Transformers. Finally, only automatic comparison metrics (e.g., BLEU) were used, while we also want to compare other aspects (human evaluation, training time and curves, etc.).

==> re_during_train.tex <==
\section{Introduction}
\begin{figure}[tb]
    \centering
    \includegraphics[width=7cm]{figures/pipeline.pdf}
    \caption{
    Our proposed pipeline. (1) A captioning model is trained on the base train set in the target language (2) and    is used to generate captions for additional images. These captions are (3) translated into English, (4) reformulated (i.e., errors are corrected while preserving correct parts of the caption are preserved), and (5) translated back into the target language. (6) The captioning model is further trained using the reformulated captions.
    }
    \label{fig:intro_image}
\end{figure}

Studies on image captioning focus, in most cases, on the English language. One of the main obstacles holding back the non-English captioning research is the lack of non-English image-caption datasets. 
Previous studies addressed this obstacle by translating English captions into the target language or transferring knowledge acquired during training on English data \gabis{What is transferring knowledge in this context? citations would help clarify}. However, translated captions are inherently different from original captions in the target language; a recent study has shown that the linguistic properties of captions translated from English to a target language are more similar to the properties of English captions than to the properties of original captions in the target language~\citep[][Appendix D]{berger-etal-2023-large} \gabis{this reference to the appendix is unclear at this point, I think the reader wouldn't know what to expect finding there}. 

This result also raises questions about the linguistic properties of captions generated by models utilizing knowledge transferred from English training \gabis{same comment about knowledge transfer being unclear}. These approaches may result in captions that are semantically similar to native captions in the non-English language, but are lexically dissimilar.\oa{is this something that you know (from previous studies or own experiments) or something that you speculate?}

We propose a data augmentation method to address the lack\oa{scarcity?} of data for non-English languages while preserving the lexical style of the language. We use the existing (small amount of) training data in the low-resource language (hereafter referred to as the \textbf{base} train set) to train a captioning model to the extent that it produces captions that are lexically similar to native captions but contain possible semantic errors (e.g., hallucinations or replacements), use it to generate captions for additional images (the \textbf{additional} train set), use an auxiliary model that corrects only semantic errors (the \textbf{reformulation} model), and use the corrected captions as additional training data for the captioning model (see Figure~\ref{fig:intro_image}). 
The reformulation model is trained to make minimal changes while correcting errors, i.e., to keep the correct parts of the caption, so that this additional training data becomes more similar lexically to the native captions in the low-resource language. \gabis{this was a bit hard for me to follow, and Fig. 1 seems also a bit complex with 6 different stages. Consider maybe putting it in a block diagram that spreads the two columns?}

We conduct experiments to better understand this novel methodology. We find that (1) a very small base train set is sufficient to generate useful\oa{are they useful for anything else but for the transfer learning protocol here?} reformulations (2K images with 5 captions each); (2) a few thousand ($\sim$ 6K) images as the base train set are sufficient for training with reformulations to lexically outperform translation-based methods, but a larger base train set would be required (> 10K images) for reformulations to semantically reach translation-based methods performance; (3) in German, when using the Multi30k dataset~\citep[][30K images, each with 5 captions]{elliott2016multi30k} as the base train set, reformulations outperform translation-based methods in the lexical metrics (BLEU -4, CIDEr) while achieving similar scores in semantic metrics (BERTScore); and (4) reformulations can be applied to any dataset of images, even without captions- and in higher efficiency compared to translation-based methods. We will make our models, data, and code available upon publication.

\gabis{IIUC, by ``lexically outperform'' we mean BLEU and similar metrics? And the conclusion is that this means that the reformulated captions are more similar in style natively written German captions? Am I correctly following the argument made in the intro? If so, I'm not sure a reviewer would be convinced that this is what BLEU numbers imply. I think that a human evaluation of their fluency or naturalness, or something like that, would be more convincing.}

\section{Background}
\subsection{Reformulations}

Several works investigated similar directions as our reformulation method.
\citet{Shen_2019_ICCV} propose a model that generates a caption and then generates a question about facts in that caption, which is answered by a human, thus applying error correction during training.
\citet{jia2020icap} propose a captioning framework where a human start generating a caption and the model reformulates it, until the human approves the generated caption.

Most similar to our work is that of \citet{ling2017teaching}, who compared training captioning models on human-generated captions with training on reformulations, showing that the second condition improved standard metrics. They focus on English and use human-generated reformulations, while we focus on utilizing model-generated reformulations for low-resource languages.

\subsection{Non-English Image Captioning}

To the best of our knowledge, all previous work on non-English image captioning has used existing English caption datasets. Studies are traditionally classified into translation methods and alignment methods.

\paragraph{Translation methods.}
The first type of studies use Machine Translation (MT) models to translate existing English captions into the low-resource language, either at train or inference time. Most work focuses on German~\cite{hitschler2016multimodal, biswas2021improving, wu2022pairs} and Chinese~\cite{li2016adding, lan2017fluency, gu2018unpaired}, although other languages have been studied, e.g., Arabic~\cite{emami2022arabic} and Assamese~\cite{nath-etal-2022-image}.

\paragraph{Alignment methods.}
The second type of studies transfer knowledge acquired during training on English data. These can be broadly be categorized into monolingual and multilingual studies. In the monolingual category, previous studies have trained a captioning model that transfers knowledge from English to one target language, such as German~\cite{elliott2015multilingual, jaffe2017generating, wu2019improving} and Japanese~\cite{miyazaki2016cross}.

In the multilingual category, a single model is trained for multiple languages. While several works~\cite{thapliyal2022crossmodal, chen2022pali} propose a joint visual encoder and a multilingual text decoder, \citet{ramos2023lmcap} propose to search the MSCOCO dataset for captions of images similar to an input image and train a multilingual language model to generate a caption in a target language given these captions as input.

Our study is the first to show that a small image-caption dataset in a low-resource language is sufficient to train an image captioning model, without utilizing any English captions.

\section{Setting}
We consider a low-resource language $L_l$ and assume a small human-annotated image-caption dataset in $L_l$ (the \textbf{base} train set) and a large set of unannotated images (the \textbf{additional} train set), some of which may have English caption annotations. We also assume the existence of an $L_l \rightarrow \text{English}$ and $\text{English} \rightarrow L_l$ translation models.

Our goal is to train a captioning model for $L_l$.
We propose to use a reformulation model as follows: Train an initial model on the base train set, use this model to generate captions for images in the additional train set, reformulate the generated captions, and continue training on the reformulated captions (Figure~\ref{fig:intro_image}).

\section{Experiments}
In this section we test our approach and compare it to different baselines. We focus on the German language.

\paragraph{Data.}
We use the Multi30k~\cite{elliott2016multi30k} train and validataion sets as the base train set, MSCOCO~\cite{lin2014microsoft} as the additional train set, and XM3600~\cite{thapliyal2022crossmodal} as the test set. Both Multi30k and XM3600 contain original captions in German. In Section~\ref{sec:entire_base_train_set} we extend the additional train set with images from ImageNet~\cite{russakovsky2015imagenet}. All data statistics are presented in Table~\ref{tab:data_statistics}.

\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\toprule
Dataset & Used for & Images & Captions \\
\midrule
Multi30k & Base & 30K & 155K \\
MSCOCO & Additional & 123K & 123K* \\
ImageNet & Additional & 1.28M & -- \\
XM3600 & Test & 3.6K & 8.6K \\
\bottomrule
\end{tabular}%
}
\caption{Statistics for the datasets used in the study. *MSCOCO contains more captions than indicated above, but we use only one caption per image for fair comparison (see \textbf{Baselines} in Section~\ref{sec:experiments}).}
\label{tab:data_statistics}
\end{table}

\paragraph{Models.}
We use the ClipCap model for its availability and size, which allow us to train it from scratch. We use the original ClipCap implementation\footnote{\href{https://github.com/rmokady/CLIP_prefix_caption}{github.com/rmokady/CLIP\_prefix\_caption}} and change the text decoder to a German version of GPT2\footnote{\href{https://huggingface.co/dbmdz/german-gpt2}{huggingface.co/dbmdz/german-gpt2}}.

In addition, we use the MarianMT models\footnote{\href{https://huggingface.co/docs/transformers/model_doc/marian}{huggingface.co/docs/transformers/model\_doc/marian}} for translation and the model described in Section~\ref{sec:reformulation_model} for reformulation. For English captioning we use the reformulation model from Section~\ref{sec:reformulation_model} with an empty input caption\footnote{We also tried using the pre-trained mPLUG checkpoint and the BLIP2 caption\_coco\_opt6.7b model, but the model from Section~\ref{sec:reformulation_model} achieved the best results.}.

\paragraph{Baselines.}
We first train an initial model (\textbf{base}) on the base train set for 10 epochs. We then consider the following models.
First, we follow the proposed reformulation pipeline: we use the \textbf{base} model to generate captions for the images in the additional train set, translate the captions into English, reformulate them, translate back to the low-resource language, and train on the resulting captions (\textbf{re}).
Additionally, to better understand the additional value of the reformulation operation, we train a model on the captions generated by \textbf{base} without reformulating them (\textbf{own}).
Finally, as translation baselines, we train a model on the translations of English human-generated (\textbf{h-tran}) and model-generated (\textbf{m-tran}) captions of the images in the additional train split. For all models except \textbf{base}, we start training from last saved checkpoint of \text{base} and train for a single epoch.

Since some of the models (\textbf{own}, \textbf{re}, \textbf{m-tran}) are based on generated captions, we only have a single caption per image, while \textbf{h-tran} can take advantage of the multiple captions per image that MSCOCO provides. To allow a fair comparison, we randomly select one caption per image for \textbf{h-tran}.

\paragraph{Metrics.}
We use the most commonly used lexical metrics for image captioning in recent years, BLEU4~\citep{papineni2002bleu} and CIDEr~\citep{vedantam2015cider}. To ensure that there is no tradeoff between lexical and semantic quality, we also use the semantic metric BERTScore~\citep{zhang2019bertscore}.

\subsection{Using a Subset of Multi30K}
To better understand the number of samples needed for efficient reformulation, we compare reformulation-based training with different sizes of base train set. We randomly select $N$ images from Multi30K for different $N$'s, and use it to train the \textbf{base} model.

\paragraph{Results.}
Results are presented in Figure~\ref{fig:subset_base_train_set}. We first note that even using only 2K images for the base train set, we obtain efficient reformulations, as the improvement of \textbf{re} over \textbf{base} is already evident for 2K images for all metrics. Moreover, we observe a consistent improvement of \textbf{re} over \textbf{own} across all metrics, demonstrating the contribution of the reformulation operation in generating quality captions for training.

Finally, we can see that at least a few thousand images are required in the base train set, so reformulation-based training (\textbf{re}) would be more efficient than translating model-generated captions (\textbf{m-tran}). This makes sense since the base model's captions are of low quality when the base train set is small, which makes the reformulations of low quality as well. We also note that, as expected, \textbf{re} matches \textbf{m-tran} faster on lexical metrics (BLEU, CIDEr- both at $\sim$6K) than on semantic metrics (BERTScore, $\sim$10K).

\begin{figure} [tb]
    \centering
    \includegraphics[width=6cm]{tables_and_plots/experiments/subset_base_train_set.png}
    \caption{Results using a subset of Multi30k as the base train set. The x-axis depicts $N$, i.e., the size of the base train set, while the y-axis depicts the metric value for each plot. All results are averaged over 3 random initializations, and the standard deviation across all models and metrics was no greater than 0.7.}
    \label{fig:subset_base_train_set}
\end{figure}

\subsection{Using the Entire Multi30K dataset} \label{sec:entire_base_train_set}
In this section, we use the entire Multi30K as the base train set, providing a solid foundation for reformulations to build upon. In addition, we explore an important advantage of reformulation-based training: Since the training data is based on captions generated from unannotated images, any dataset with unannotated images can be used as training data. We use the ImageNet dataset~\citep{russakovsky2015imagenet}, a common dataset for training image classification models. We use the common subset ILSVRC, which contains 1.28 million images without captions.

We train 3 additional models, one for each generated-caption based method (\textbf{m-tran+IN}, \textbf{own+IN}, \textbf{ours+IN}) where in addition to MSCOCO, we add the images from ImageNet to the additional train set, increasing the number of images in the additional train set to 1.4 million. We do not train such a model for the \textbf{h-tran} baseline, since it is based on translated human-generated captions, which are not available for ImageNet.

\paragraph{Results.}
Results are presented in Table~\ref{tab:entire_base_train_set}. When using MSCOCO as the additional train set, we observe that \textbf{re} outperforms all other methods in the lexical metrics (B@4 and CIDEr), while the model-generated translated captions baseline (\textbf{m-tran}) achieves the best result in the semantic metric BERTScore, although \textbf{re} achieves the second best result with 0.4 points less than \textbf{m-tran}.

\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc}
\toprule
 & B@4 & CIDEr & BS \\
\midrule
base & 2.2 $\pm$ 0.1 & 11.8 $\pm$ 0.5 & 71.9 $\pm$ 0.0 \\
\midrule
h-tran & 1.9 $\pm$ 0.2 & 15.1 $\pm$ 0.8 & 72.2 $\pm$ 0.4 \\
m-tran & 2.6 $\pm$ 0.1 & 16.2 $\pm$ 0.7 & \textbf{72.9 $\pm$ 0.3} \\
own & 2.3 $\pm$ 0.1 & 12.6 $\pm$ 0.4 & 71.9 $\pm$ 0.1 \\
re & \textbf{2.9 $\pm$ 0.3} & \textbf{16.9 $\pm$ 0.6} & 72.5 $\pm$ 0.3 \\
\midrule
m-tran+IN & 3.2 $\pm$ 0.2 & 20.1 $\pm$ 0.3 & 73.2 $\pm$ 0.1 \\
own+IN & 2.2 $\pm$ 0.2 & 12.5 $\pm$ 0.3 & 71.7 $\pm$ 0.2 \\
re+IN & \textbf{3.7 $\pm$ 0.1} & \textbf{21.4 $\pm$ 0.1} & \textbf{73.4 $\pm$ 0.1} \\
\bottomrule
\end{tabular}%
}
\caption{Results for training on the entire base train set, on the Crossmodal 3600 dataset. \textbf{base} is trained only on the base train set, \{\textbf{h-tran, m-tran, own, re}\} are trained on the base train set and then on MSCOCO as the additional train set, and the \textbf{+IN} models are trained on the base train set and then on MSCOCO + ImageNet as the additional train set. All results are averaged over 3 random initializations. The best result for each metric is shown in bold.}
\label{tab:entire_base_train_set}
\end{table}

When using a large additional train set (MSCOCO + ImageNet), the lexical gap between \textbf{re} and \textbf{m-tran} increases (0.5 B@4 points and 1.3 CIDEr points), while on the semantic BERTScore metric \textbf{re} actually outperforms \textbf{m-tran}. This is a promising result for training models at scale with large non-annotated image datasets using reformulation-based captions.

To put our results in the context of current published models, we compare our best model (\textbf{re+IN}) with the models presented in the original XM3600 paper~\cite{thapliyal2022crossmodal}, which represent the current published state-of-the-art on XM3600 in German\footnote{We recognise that the PaLI model~\cite{chen2022pali} likely outperforms the models in the XM3600 paper, as they report significant improvement over these models in 7 different languages (Table 2 in the PaLI paper). However, they didn't report results for German.}. Results are shown in Table~\ref{tab:comparison_to_xm3600}; the only model that outperforms our model is BB+CC, trained on captions from MSCOCO and Conceptual Captions~\cite{sharma2018conceptual} translated from English into 35 different languages, summing up to $>3$M image-caption pairs only in German. All other models (BB, Lg, Bg) are trained on MSCOCO caption translated into 35 languages.

\begin{table}[!t]
\centering
\begin{tabular}{cc}
\toprule
Model & CIDEr \\
\midrule
BB & 11.2 \\
Lg & 13.0 \\
Bg & 13.8 \\
BB+CC & 22.4 \\
\midrule
re+IN & 21.4 \\
\bottomrule
\end{tabular}
\caption{Comparison between our best model and the models presented in \citet{thapliyal2022crossmodal}. The BB, Lg, and Bg models are trained on 35X(123K, 616K) image-translated caption pairs, of which (123K, 616K) are in German. BB+CC is trained on 35X(3.4M, 3.9M) image-translated caption pairs, of which (3.4M, 3.9M) are in German. re+IN is trained on (30K, 155K) image-original German caption pairs and then on 1.4M unannotated images.}
\label{tab:comparison_to_xm3600}
\end{table}


==> tables_and_plots/experiments/comparison_to_xm3600.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{cc}
\toprule
Model & CIDEr \\
\midrule
BB & 11.2 \\
Lg & 13.0 \\
Bg & 13.8 \\
BB+CC & 22.4 \\
\midrule
re+IN & 21.4 \\
\bottomrule
\end{tabular}
\caption{Comparison between our best model and the models presented in \citet{thapliyal2022crossmodal}. The BB, Lg, and Bg models are trained on 35X(123K, 616K) image-translated caption pairs, of which (123K, 616K) are in German. BB+CC is trained on 35X(3.4M, 3.9M) image-translated caption pairs, of which (3.4M, 3.9M) are in German. re+IN is trained on (30K, 155K) image-original German caption pairs and then on 1.4M unannotated images.}
\label{tab:comparison_to_xm3600}
\end{table}


==> tables_and_plots/experiments/data_statistics.tex <==
\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\toprule
Dataset & Used for & Images & Captions \\
\midrule
Multi30k (train) & Base model & 30K & 150K \\
MSCOCO & Translation & 123K & 616K \\
Multi30k (test) & Test & 1K & 5K \\
% XM3600 & Test & 3.6K & 8.6K \\
\bottomrule
\end{tabular}%
}
\caption{Statistics for the datasets used in the study.}
\label{tab:data_statistics}
\end{table}


==> tables_and_plots/experiments/german_xm3600_results.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{c|cc}
\toprule
 & B@4 & CIDEr \\
\midrule
base & 2.2 $\pm$ 0.1 & 11.8 $\pm$ 0.5 \\
tran & 1.9 $\pm$ 0.2 & 15.1 $\pm$ 0.8 \\
% m-tran & 2.6 $\pm$ 0.1 & 16.2 $\pm$ 0.7 \\
base+re & \textbf{4.4 $\pm$ 0.2} & \textbf{26.2 $\pm$ 0.2} \\
\midrule
BB & -- & 11.2 \\
Lg & -- & 13.0 \\
Bg & -- & 13.8 \\
BB+CC & -- & 22.4 \\
\bottomrule
\end{tabular}
\caption{Results on the XM3600 dataset. All results for our experiments (upper part) are averaged over 3 random initializations. Training on Multi30k and reformulating (in bold) ourperforms all other methods.}
\label{tab:german_xm3600_results}
\end{table}


==> tables_and_plots/experiments/re_during_inference_spice_blip.tex <==
\begin{table}[!t]
\small
\centering
\begin{tabular}{cccccrc}
\toprule
 & Obj & Rel & Att & Car & Siz & Col \\
\toprule
MSCOCO & 1.9 & 1.1 & 7.2 & 5.7 & 6.7& 16.8\\
Flickr30k & 1.5 & 2.2 & 5.5 & 8.3 & -3.6 & 14.5 \\

% & 1.50\% \\
% Relation   \\
% Attribute  \\
% Cardinality  & 8.26\% \\
% Size  & -3.61\% \\
% Color  & 14.54\% \\
\bottomrule
\end{tabular}
\caption{Performance change after reformulation of BLIP outputs on SPICE elements relative to  performance before reformulation (in \%).}
\label{tab:re_during_inference_spice}
\end{table}


% \begin{table}[!t]
% \small
% \centering
% \begin{tabular}{ccc}
% \toprule
% & MSCOCO & Flickr30k \\
% \toprule
% Object & 1.89\% & 1.50\% \\
% Relation & 1.06\% & 2.18\% \\
% Attribute & 7.20\% & 5.53\% \\
% Cardinality & 5.69\% & 8.26\% \\
% Size & 6.69\% & -3.61\% \\
% Color & 16.84\% & 14.54\% \\
% \bottomrule
% \end{tabular}
% \caption{Performance improvement/decrease after reformulation of BLIP outputs on SPICE elements, in percentage (out of the recorded performance before reformulation).}
% \label{tab:re_during_inference_spice}
% \end{table}

